UFOGen: You Forward Once Large Scale Text-to-Image Generation via Diffusion GANs

Text-to-image diffusion models have demonstrated remarkable capabilities in transforming textual prompts into coherent images, yet the computational cost of their inference remains a persistent challenge. To address this issue, we present UFOGen, a novel generative model designed for ultra-fast, one-step text-to-image synthesis. In contrast to conventional approaches that focus on improving samplers or employing distillation techniques for diffusion models, UFOGen adopts a hybrid methodology, integrating diffusion models with a GAN objective. Leveraging a newly introduced diffusion-GAN objective and initialization with pre-trained diffusion models, UFOGen excels in efficiently generating high-quality images conditioned on textual descriptions in a single step. Beyond traditional text-to-image generation, UFOGen showcases versatility in applications. Notably, UFOGen stands among the pioneering models enabling one-step text-to-image generation and diverse downstream tasks, presenting a significant advancement in the landscape of efficient generative models.

==> sec/experiments_arxiv.tex <==
\section{Experiments}
In this section, we evaluate our proposed UFOGen model for the text-to-image synthesis problem. In Section \ref{sec exp t2i}, we start with briefly introducing our experimental setup, followed by comprehensive evaluations of UFOGen model on the text-to-image task, both quantitatively and qualitatively. We conduct ablation studies in Section \ref{sec exp ablation}, highlighting the effectiveness of our modifications introduced in Section \ref{sec_method}. In Section \ref{sec exp app}, we present qualitative results for downstream applications of UFOGen. 

\subsection{Text-to-image Generation}\label{sec exp t2i}
\vspace{2mm} \noindent \textbf{Configuration for Training and Evaluation} For experiments on text-to-image generation, we follow the scheme proposed in Section \ref{sec_method scale up} to initialize both the generator and discriminator with the pre-trained Stable Diffusion 1.5\footnote{\url{https://huggingface.co/runwayml/stable-diffusion-v1-5}} model ~\cite{rombach2022high}. We train our model on the LAION-Aesthetics-6+ subset of LAION-5B \cite{schuhmann2022laion}. More training details are provided in Appendix \ref{app exp details}. For evaluation, we adopt the common practice that uses zero-shot FID \cite{heusel2017gans} on MS-COCO ~\cite{lin2014microsoft}, and CLIP score with ViT-g/14 backbone \cite{radford2021learning}. 

\vspace{2mm} \noindent \textbf{Main Results} To kick-start our evaluation, we perform a comparative analysis in Table \ref{tab:full-5k}, bench-marking UFOGen against other few-step sampling models that share the same Stable Diffusion backbone. Our baselines include Progressive Distillation \cite{meng2023distillation} and its variant \cite{li2023snapfusion}, which are previously the state-of-the-art for few-step sampling of SD, as well as the concurrent work of InstaFlow \cite{liu2023insta}. Latent Consistency Model (LCM) \cite{luo2023latent} is excluded, as the metric is not provided in their paper. Analysis of the results presented in Table \ref{tab:full-5k} reveals the superior performance of our single-step UFOGen when compared to Progressive Distillation across one, two, or four sampling steps, as well as the CFG-Aware distillation \cite{li2023snapfusion} in eight steps. Furthermore, our method demonstrates advantages in terms of both FID and CLIP scores over the single-step competitor, InstaFlow-0.9B, which share the same network structure of SD with us. Impressively, our approach remains highly competitive even when compared to InstaFlow-1.7B with stacked UNet structures, which effectively doubles the parameter count.

% \paragraph{Training Cost}
\begin{table}[t]
\scriptsize
    \centering
    \begin{tabular}{lcccc}
    \toprule
    Method  & \#Steps & Time (s) & FID-5k & CLIP \\ \midrule
    \multirow{2}{*}{DPM Solver~\cite{lu2022dpm}} & 25 & 0.88  & \textbf{20.1}  & 0.318  \\ 
     & 8 & 0.34  &  31.7 & \textbf{0.320}  \\ 
    \midrule
    \multirow{3}{*}{Progressive Distillation~\cite{meng2023distillation}} &1 & 0.09 & 37.2 & 0.275 \\ 
    & 2 & 0.13  & 26.0 & 0.297  \\
    & 4 & 0.21  & 26.4 & 0.300 \\  \midrule
    CFG-Aware Distillation~\cite{li2023snapfusion} & 8& 0.34 & 24.2 & 0.30 \\
    \midrule 
    InstaFlow-0.9B & 1 & 0.09 & 23.4  &0.304  \\
    InstaFlow-1.7B & 1 & 0.12 & \textbf{22.4}  & 0.309 \\
    \midrule
    \textbf{UFOGen} & 1 & 0.09  & 22.5  & \textbf{0.311} \\
    \bottomrule
    \end{tabular}
    \caption{Comparison of FID on MSCOCO-2017 5k and CLIP score. All models are based on SD. Numbers of progressive distillation and InstaFlow are cited from \cite{liu2023insta}.
    }
    \label{tab:full-5k}
\end{table}

\input{sec/figure_tables/main_compare}

The results depicted in Table \ref{tab:full-5k} may suggest that InstaFlow remains a strong contender in one-step generation alongside UFOGen. However, we argue that relying solely on the MS-COCO zero-shot FID score for evaluating visual quality might not be the most reliable metric, a concern highlighted in prior research such as \cite{podell2023sdxl,kirstain2023pick} and discussed by \cite{betzalel2022study}. % An evident example of this concern is that Stable Diffusion models obtain the lowest FID  when employing a guidance scale $3.0$, however, in practice, much larger guidance scales are commonly employed to attain higher quality. 
Consequently, we believe that qualitative assessments can provide more comprehensive insights. We present qualitative comparisons involving InstaFlow and LCM\footnote{InstaFlow (\url{https://huggingface.co/spaces/XCLiu/InstaFlow}) and LCM (\url{https://huggingface.co/spaces/SimianLuo/Latent_Consistency_Model})} in Table \ref{tab:main_comparison}. The comparisons allow for a clear-cut conclusion: UFOGen's one-step image generation surpasses InstaFlow by a substantial margin in terms of image quality. Notably, UFOGen also demonstrates significant advantages when contrasted with the 2-step LCM, as showed by the evident blurriness present in LCM's samples. Furthermore, even when compared to the samples generated by the 4-step LCM, our generated images exhibit distinct characteristics, including sharper textures and finer details. We do not present results of single-step LCM, as we observe that it fail to generate any textures (see Appendix \ref{app failed lcm-1}). Additional examples of the comparison are provided in Appendix \ref{app extra comparison}, where we display multiple images generated by each model for different prompts. We provide additional qualitative samples of UFOGen in Appendix \ref{app extra t2i results}.

\begin{table}[t]
    \centering
    \begin{tabular}{lcccl}
    \toprule
     Method & Type & Time (s) & \# Param. & FID-30k \\ \midrule
     DALLE~\cite{ramesh2021zero} & AR  &- & 12B & 27.5 \\ 
    Parti-20B~\cite{yu2022scaling} & AR  &- & 20B & 7.23 \\ 
    Make-A-Scene~\cite{gafni2022make} & AR  &25.0 & - & 11.84 \\ \midrule
    GLIDE~\cite{nichol2022glide} &  Diff  &  15.0 & 5B & 12.24 \\
    DALLE 2~\cite{ramesh2022hierarchical} & Diff  &  - & 5.5B & 10.39 \\
    Imagen~\cite{ho2022imagen} &  Diff  & 9.1 & 3B & 7.27 \\
    eDiff-I~\cite{balaji2022ediffi} &  Diff  & 32.0 & 9B & 6.95 \\
    SD~\cite{rombach2022high} &  Diff  & 2.9 & 0.9B & 9.62 \\ \midrule
    LAFITE~\cite{zhou2022towards} & GAN  & 0.02 & 75M & 26.94 \\    
    StyleGAN-T~\cite{sauer2023stylegan} & GAN  & 0.10 & 1B & 13.90 \\
    GigaGAN~\cite{kang2023scaling} & GAN  & 0.13 & 1B & 9.09 \\ \midrule
    Muse-3B~\cite{chang2023muse} & - &  1.3 & 3B & 7.88 \\    
    InstaFlow~\cite{liu2023insta}& - &  0.09&0.9B&13.10\\
    \midrule
    \textbf{UFOGen (Ours)} & -  & 0.09 & 0.9B & 12.78 \\
    \bottomrule
    \end{tabular}
    \caption{Comparison of FID on MSCOCO 2014 with 30k images. Numbers of other models are cited from \cite{liu2023insta}. Inference time measurement follows the setting of \cite{gigagan}.}
    \label{tab:full-30k}
\end{table}

For completeness, we extend our comparison to encompass a diverse array of text-to-image generative models in Table \ref{tab:full-30k}. While the results in Table \ref{tab:full-30k} are not directly comparable due to substantial variations in model architecture, parameter count, and training data, it is noteworthy that UFOGen is a competitive contender among the contemporary landscape of text-to-image models, offering the advantage of remarkable speed over auto-regressive or diffusion models, thanks to its inherent one-step generation capability.

Based on both quantitative and qualitative assessments, we assert that UFOGen stands as a powerful text-to-image generative model, capable of producing sharp and visually appealing images that align well with the provided text conditioning, all in a single step. Our evaluation underscores its capacity to produce superior sample quality when contrasted with competing diffusion-based methods designed for a few-step generation process. 
% Moreover, in the broader context of model comparison, UFOGen achieves a favorable position within the trade-off between quality and inference time.

% \paragraph{Training Cost} We would like to highlight another advantage of of model, which is the low training cost. We observe that when adopting the Stable Diffusion initialization introduced in Section \ref{sec_method scale up}, training of UFOGen converges extremely fast. 

\subsection{Ablation Studies}\label{sec exp ablation}
Ablation studies have been conducted to offer deeper insights into the effectiveness of our training strategies. As outlined in Table~\ref{tab:main_ablation}, we compare the training of diffusion-GAN hybrid models using the SIDDM objective \cite{ssidms} against the proposed UFOGen objective in Section \ref{sec_method one step}. The results validate our assertions, demonstrating that the modifications in the UFOGen objective facilitate one-step sampling. 
% We additionally provide qualitative samples, and an supplementary ablation study on the denoising step size during training in Appendix \ref{app extra ablation}.

\begin{table}[t]
    \centering
    \begin{tabular}{lccc}
    \toprule
    Method & \#Steps  & FID-5k & CLIP \\ \midrule
    \multirow{2}{*}{SIDDM~\cite{ssidms}} & 4 & 21.7 & 0.306 \\
      & 1  & 28.0 & 0.289 \\\midrule
    \multirow{2}{*}{UFOGen} & 4 & 22.1  & 0.307 \\
    & 1 & 22.5 & 0.311 \\
    \bottomrule
    \end{tabular}
    \caption{Ablation study comparing the SIDDM objective with our UFOGen objective, incorporating the introduced modifications detailed in Section \ref{sec_method one step}.
    }
    \label{tab:main_ablation}
\end{table}

\subsection{Applications}\label{sec exp app}
A promising aspect of text-to-image diffusion models is their versatility as foundational components for various applications, whether fine-tuned or utilized as is. In this section, we showcase UFOGen's ability to extend beyond text-to-image generation, while benefiting from its unique advantage of single-step generation. Specifically, we explore two applications of UFOGen: image-to-image \cite{meng2021sdedit} generation and controllable generation \cite{zhang2023adding, mou2023t2i}.
\input{sec/figure_tables/main_i2i}

Table \ref{tab:main_i2i} showcases UFOGen's image-to-image generation outcomes. Following SDEdit \cite{meng2021sdedit}, we introduce a suitable amount of noise to the input data, and let UFOGen to execute single-step generation based on the given prompt. Our observations affirm that UFOGen adeptly produces samples that adhere to the specified conditions of both the prompt and the input image. 

To facilitate controllable generation, we conduct fine-tuning of UFOGen by incorporating an additional adapter network, akin to the approach outlined in \cite{mou2023t2i}. This adapter network takes control signals as input to guide the generation process. In our exploration, we employ two types of control signals: depth maps and canny edges. The results are presented in Table \ref{tab:main_control}. Post fine-tuning, UFOGen exhibits the ability to generate high-quality samples that align with both the provided prompt and control signal.

Our results highlight UFOGen can work on diverse generation tasks in a single step, a distinctive feature that, to the best of our knowledge, sets our model apart. Unlike GAN-based text-to-image models \cite{sauer2023stylegan,kang2023gigagan}, which lack the ability to handle zero-shot image-to-image generation tasks as they do not generate samples through denoising, UFOGen excels in this context. Moreover, our model succeeds in controllable generation, a domain that earlier GAN-based models have not explored due to the complexities of fine-tuning and adding supplementary modules to the StyleGAN architecture. Consequently, the flexibility of our model in addressing various downstream tasks positions it uniquely among one-step text-to-image models. 
% Additional results of the applications are provided in Appendix \ref{app extra application}.

